Vision-Based Uncertainty-Aware Motion Planning based on Probabilistic Semantic Segmentation

For safe operation, a robot must be able to avoid collisions in uncertain environments. Existing approaches for motion planning under uncertainties often assume parametric obstacle representations and Gaussian uncertainty, which can be inaccurate. While visual perception can deliver a more accurate representation of the environment, its use for safe motion planning is limited by the inherent miscalibration of neural networks and the challenge of obtaining adequate datasets. To address these limitations, we propose to employ ensembles of deep semantic segmentation networks trained with massively augmented datasets to ensure reliable probabilistic occupancy information. To avoid conservatism during motion planning, we directly employ the probabilistic perception in a scenario-based path planning approach. A velocity scheduling scheme is applied to the path to ensure a safe motion despite tracking inaccuracies. We demonstrate the effectiveness of the massive data augmentation in combination with deep ensembles and the proposed scenario-based planning approach in comparisons to state-of-the-art methods and validate our framework in an experiment with a human hand as an obstacle.

==> figs/intro_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figs/intro_fig.pdf}
    \caption{Our framework combines visual perception with safe motion planning. By applying systematic data augmentation and an ensemble scheme to semantic segmentation, we obtain reliable probabilistic occupancy information in uncertain environments. Based on the perception data, we plan a chance-constrained path and a maximum velocity profile such that safety of the real robot motion is ensured despite possible tracking errors.}
    \label{fig:intro_fig}
\end{figure}

==> figs/planning_hand.tex <==
\begin{figure}
% \includegraphics[width=\linewidth]{data/path_hand.jpg}
\centering
\includegraphics[width=0.8\linewidth]{data/path_hand_small.jpg}
\captionof{figure}{Approximating the hand with many simple geometries and assuming zero uncertainty leads to roughly similar paths for the different methods. However, the procedure is tedious and being less accurate worsens path quality.}
\label{fig:planning_hand}
\end{figure}
